IceCube-Gen2: A Vision for the Future of Neutrino Astronomy in Antarctica

The recent observation by the IceCube neutrino observatory of an astrophysical flux of neutrinos represents the "first light" in the nascent field of neutrino astronomy. The observed diffuse neutrino flux seems to suggest a much larger level of hadronic activity in the non-thermal universe than previously thought and suggests a rich discovery potential for a larger neutrino observatory. This document presents a vision for an substantial expansion of the current IceCube detector, IceCube-Gen2, including the aim of instrumenting a $10\,\mathrm{km}^3$ volume of clear glacial ice at the South Pole to deliver substantial increases in the astrophysical neutrino sample for all flavors. A detector of this size would have a rich physics program with the goal to resolve the sources of these astrophysical neutrinos, discover GZK neutrinos, and be a leading observatory in future multi-messenger astronomy programs.

==> beyondsm.tex <==

IceCube has been extremely successful in searches for dark matter and other physics topics beyond the Standard
Model~\cite{Aartsen:2012kia,Abbasi:2011eq,Aartsen:2013dxa}. Plans for the low-energy extension of IceCube will extend the possibility
of such searches to energies at the few GeV region~\cite{Aartsen:2014oha}. However, some of the current searches in IceCube will benefit
from an extended array.

On the dark matter side, scenarios in which particles are heavy become testable. Dark Matter searches with neutrinos have
traditionally focused on scenarios motivated to test the Weakly Interacting Massive Particle (WIMP) hypothesis, by looking
for dark matter captured in the Sun~\cite{Aartsen:2012kia}, Earth, or from annihilations in the galactic
halo~\cite{Abbasi:2011eq,Aartsen:2014hva} or galaxy clusters.  But dark matter candidates with a mass beyond the WIMP
scale of a few GeV to TeV could be non-thermally produced in the early universe. Annihilations or decays of such particles
are most effectively probed with high-energy neutrinos in indirect searches from the galactic halo or galactic center.
Given their ability to travel long distances without attenuation, neutrinos offer excellent prospects for the detection
of high mass dark matter~\cite{Rott:2014kfa,Murase:2012xs}. Dark matter lifetimes exceeding $10^{28}$~s could be tested for
decay modes of $\chi \rightarrow \nu X$.\par

A bigger detector additionally opens new analysis possibilities for exotica that are not a viable option for even a cubic-
kilometer array like IceCube. The detailed characterization of the recently discovered astrophysical neutrino flux provides
a unique window to physics beyond the Standard Model on topics ranging from new particle searches to
effects due to extra dimensions.  These opportunities include searches for extremely bright events, such as 
magnetic monopoles\cite{Aartsen:2014awd}, for Lorentz invariance from neutrino 
bremsstrahlung\cite{Borriello:2013ala}, for evidence of TeV gravity models and extra dimensions\cite{Kowalski:2002gb,AlvarezMuniz:2002ga,Anchordoqui:2006fn,Illana:2006mv},
for heavy sterile neutrino decay\cite{Mauricio:14a}, or evidence of physics beyond the standard model
in the extremely high energy atmospheric neutrino interactions\cite{Illana:2007ra,Illana:2005pu,Albuquerque:2006am,Reynoso:2007zb}. 

